Time Reversal Symmetry for Efficient Robotic Manipulations in Deep Reinforcement Learning

Symmetry is pervasive in robotics and has been widely exploited to improve sample efficiency in deep reinforcement learning (DRL). However, existing approaches primarily focus on spatial symmetries, such as reflection, rotation, and translation, while largely neglecting temporal symmetries. To address this gap, we explore time reversal symmetry, a form of temporal symmetry commonly found in robotics tasks such as door opening and closing. We propose Time Reversal symmetry enhanced Deep Reinforcement Learning (TR-DRL), a framework that combines trajectory reversal augmentation and time reversal guided reward shaping to efficiently solve temporally symmetric tasks. Our method generates reversed transitions from fully reversible transitions, identified by a proposed dynamics-consistent filter, to augment the training data. For partially reversible transitions, we apply reward shaping to guide learning, according to successful trajectories from the reversed task. Extensive experiments on the Robosuite and MetaWorld benchmarks demonstrate that TR-DRL is effective in both single-task and multi-task settings, achieving higher sample efficiency and stronger final performance compared to baseline methods.

==> final_remarks.tex <==
\section{Final Remarks}
To facilitate the authors’ response to any final questions and comments from the reviewers, we have decided to provide an “Author Final Remarks” response mechanism.

This 2500-character \textcolor{red}{non-editable} field is optional, and allows authors to convey any final pressing comments relevant to the rebuttal or discussions. It is primarily intended for the AC’s consideration during decision-making, but it is also visible to reviewers to support internal discussions. \textcolor{red}{Please note that reviewers, ACs, and SACs will not be able to respond to the remarks in this field - the mechanism is intended as a final response providing closure to Author-Reviewer discussions.} While \textcolor{red}{the hard deadline is Aug 15 AoE}, we recommend authors to convey any final remarks, responses and conclusions they may have as soon as possible to ensure the AC has sufficient opportunity to take them into account.

Answer:
{
We would like to thank all the reviewers for their efforts in reviewing our paper and providing us with helpful feedback.

Our work explores how to exploit temporal symmetry in deep RL, an underexplored direction compared to spatial symmetry.
The reviewers noted several positive aspects of our submission.
Time reversal symmetry occurs frequently in real-world robotics, showcasing its practical relevance (Reviewer TdWt).
Our main contribution is to show that our proposed techniques with time reversal symmetry are effective in improving data efficiency of deep RL.
Our two proposed techniques, trajectory reversal augmentation and time-reversal guided reward shaping, are technically sound (Reviewer fKuw).
Simultaneously, our method is described as the "shortest path" solution to an effective method (Reviewer Pawe) and praised for its intuitiveness and broad applicability (Reviewer dzfv).
The results in simulation environments are compelling (Reviewer dzfv), demonstrating robustness to hyperparameter choices and consistent performance gains from each proposed technique (Reviewer TdWt).
Crucially, our ablation studies precisely isolate each proposed technique and prove the necessity of each component (Reviewer Pawe).

During the rebuttal process, we have thoroughly answered the questions raised by each reviewer.
Specifically, we have included additional experimental results requested by Reviewer TdWt (Question1) and Reviewer Pawe (Question2), strengthening our validation.
Also, we have improved the writing of our paper for better readability and logic flow, thanks to detailed suggestions proposed by reviewer TdWt.

Finally, we agree that real-world experimental validation would be important.
However, our work is a first step to demonstrate how to effectively exploit time reversal symmetry in deep RL methods.
We leave this real-world validation to future work.

% \todo{improve here, write the reviewers in ()}
% Our current work explores how to exploit temporal symmetry in deep RL, an underexplored direction compared to spatial symmetry.
% Time reversal symmetry occurs frequently in real-world robotics, showcasing the practical relevance of this direction (reviewer TdWt).
% % As noted by reviewer TdWt, time reversal symmetry occurs frequently in real-world robotics, showcasing the practical relevance of this direction.
% Our main contribution is to show that our proposed techniques with time reversal symmetry are effective in improving data efficiency of deep RL.
% Reviewer fkuw confirmed the technical soundness of our two proposed techniques, trajectory reversal augmentation and time reversal guided reward shaping. 
% Simultaneously, Reviewer Pawe praised the elegance of our proposed techniques as the "shortest path" solution to an effective method.
% Reviewer dzfv endorsed the intuitiveness of our idea and broad applicability of our method.
% The results in simulation environments are compelling (Reviewer dzfv), demonstrating robustness to hyperparameter choices and consistent performance gains from each proposed technique (Reviewer TdWt).
% As highlighted by Reviewer Pawe, our ablation studies precisely isolate each proposed technique and prove the necessity of each component.

% Reviewer fkuw: The two proposed techniques—trajectory reversal augmentation and time reversal guided reward shaping—are well thought out and methodically sound. The dynamics-consistent filter for ensuring valid reversed transitions is an excellent addition.
% Reviewer TdWt: Partial time reversal symmetry appears in many real world robotics, so the topic is relevant and practically useful.
% Reviewer Pawe: This work in particular is impressive in that it takes a simple idea, and with proper evaluation, shows that it leads to improvement in some real benchmark tasks. The idea is sensible, and the method design that leads around the idea feels like the "shortest path" needed to reach the effective method, which is desirable and yet rare in recent works. The ablation studies presented in the paper are also sensible, and does the ablations at the right level of abstraction to prove the necessity of each of the pieces.
% Reviewre dzfv:
% I liked the main idea of the paper. I liked that it was intuitive. This seems like an approach that should be helpful in a variety of situations.
% I thought that the methods that were proposed were pretty reasonable and the experimental results indicate that they are generally helpful.
% I thought the experiments were good. I was convinced.
}

==> rebuttal.tex <==
\section{Rebuttal}
\subsection{Reviewer fKuw}
\jypmodify{Thank you for indicating our contributions and providing thoughtful feedback on our work.}

\hjsmodify{In this work, we focus on robotics tasks with time reversal symmetry, and evaluate our proposed method in simulation. 
We definitely agree that applying our approach in a real-world setting is an important step to prove the effectiveness of our method for solving those time-symmetric robotics tasks.
And it is an interesting direction to learn the temporal symmetry if it does not obviously exist in tasks.
We leave the real-world experiments and learning temporal symmetry as future work.}

\jypmodify{Below, we answer each question in detail.}
\begin{itemize}
    \item Weakness:
    \begin{enumerate}
        \item Lack of Real-World Experiments: While the paper provides extensive simulation-based experiments, the lack of real-world robotic evaluations is a key limitation. This is particularly relevant in robotics, where simulations often fail to capture real-world complexities such as sensor noise, physical dynamics, and actuator constraints.

        \item Generalization to Other Domains: The proposed methods are shown to work in robotics, but it is unclear how easily these techniques might generalize to other domains, such as those that do not have clear time reversal symmetry.

        \item Complexity: While the proposed methods are valuable, they introduce additional complexity into the reinforcement learning setup, such as the need for inverse dynamics models and filtering. The practical implementation of these components could be challenging in some settings.
    \end{enumerate}

    \item Questions:
    \begin{enumerate}
        \item Can the time reversal symmetry techniques be applied to a wider range of robotic tasks, or are they limited to tasks with explicitly reversible actions (e.g., peg insertion/removal)? It would be helpful if the authors could provide insight into how broadly these methods could be applied.

        Answer:
        % \jypmodify{
        % % Thank you for raising the critical question about applicability of our method beyond explicitly reversible actions.
        % We would like to clarify that our method
        % also take advantage of partially reversible transitions.}
        \hjsmodify{We would like to clarify that our method exploits two types of symmetry: full time reversal symmetry (FTR) and partial time reversal symmetry (PTR). 
        Peg insertion/removal and door opening/closing inward are examples of FTR and PTR task pairs respectively.}
        \jypmodify{In door opening/closing inward, most reversed transitions are filtered out by the dynamics-consistent filter, since the agent cannot reverse the action (i.e., from "push the door" to "grasp the handle and pull the door") without first grasping the handle.}
        \jypmodify{The detailed examples of partial reversibility can be found in Example 2 of Section 4.1.}
        \jypmodify{
        We design a time reversal reward shaping mechanism to handle these partially reversible transitions.
        A potential model is trained with successful trajectories of task A and used to guide the agent training of task B through potential-based reward shaping, as detailed in Section 4.3.
        }

        \item (not sure about the answer) Given that the paper does not include real-robot evaluations, how confident are the authors that their approach will perform well in a physical robot, particularly in environments with noise or variability in actuator performance? Future work could explore bridging this gap between simulation and real-world testing.

        Answer: 
        % \jypmodify{
        % % Thank you for raising an important consideration about real-world deployment.
        % Our experiments show enhanced sample efficiency and final performance within simulated environments, suggesting that our approach can effectively facilitate the learning process during the simulation phase for those aiming to deploy robots using the sim-to-real workflow.
        % Moreover, we fully agree that future research could explore how to apply time reversal symmetry to data purely obtained from real-world scenarios and potentially integrate this idea with imitation learning methods such as diffusion policy.}
        \hjsmodify{As stated at the beginning of the response, we admit the significance of real-world experiments and leave it as future work. 
        Considering the difficulties of conducting RL directly under real-world setting, a common practice is to train the policy with RL in simulation and deploy the policy in real-world by solving the sim-to-real gap.
        Our approach can effectively facilitate the learning process during the simulation phase.}

        \item In partially reversible tasks, how does the agent handle situations where only certain components of the state are reversible (e.g., door state vs. robot state)? A more detailed explanation of how partial reversibility impacts training would be useful.

        Answer: \jypmodify{
        For tasks where only subsets of states exhibit time reversal symmetry, reversed trajectories obtained from trajectory reversal augmentation often violate true environment dynamics, leading to low quality data that may even hurt agent training.
        Instead, our method leverages time reversal guided reward shaping to exploit the partial reversibility.} 
        \hjsmodify{Intuitively, for a high-reward trajectory from one task (door from open to closed), if a trajectory from another task can achieve the reversed object states (door from closed to open), it should likewise receive a high reward.}
        \jypmodify{
        % If the agent receives a high-reward trajectory $(s_0, s_1, ..., s_n)$ for task A, the agent should likewise receive a high reward if it achieves the reversed sequence $(x_n, ..., x_1, x_0)$ in task B, where $x_t$ denote the object-related component of the full state $s_t$.
        This motivates us to employ reward shaping to guide the RL agent with these partially reversible transitions}
        \hjsmodify{, as detailed in Section 4.3.}
        \jypmodify{
        Furthermore, we choose to use potential-based reward shaping as it preserves policy optimality and train a potential model so that we can fully utilize all successful trajectories.}
        % The potential model can guide the agent training through potential-based reward shaping.}
        % , as detailed in Section 4.3.
        % Furthermore, Figure 4 quantitatively demonstrates the performance gains achieved through our proposed time reversal guided reward shaping technique. 
        % To rigorously validate design choices of this technique, we also conduct an ablation study, as detailed in Section 5.2. 
        % }
    \end{enumerate}
\end{itemize}

\subsection{Reviewer TdWt}
\jypmodify{Thank you for summarizing our work and providing thoughtful feedback that helps us strengthen both the presentation and technical depth of our paper.
Below we answer your questions in detail.}
\begin{itemize}
    \item Weakness:
    \begin{enumerate}
        \item Baselines. TR-DRL is the only method that leverages this knowledge and thus naturally has an advantage over vanilla baselines. I wouldn't say this is necessarily an unfair advantage, though; a core contribution of this paper is showing the benefit of incorporating knowledge of time reversal into training. However, I think some discussion is warranted on other ways we could potentially leverage this information. e.g. learning reversible action representations [1]. To rephrase my comment: Experiments show that adding time-reversed augmentated data to the replay buffer improves data efficiency. Are there other ways to integrate time-reversal information? How do they compare?

        \item Time reversal examples are a bit unclear. My understanding other partial time reversal is rooted in my understanding of locally factored dynamics discussed by Pitis et. al. [2] (see the next section below for additional context). I had a bit of trouble understanding what Example 2 was talking about until I made this connection. Are we saying that the door state is reversible because there exists some action that can reverse the door's trajectory?

        \item Mild impact. The paper addresses a very specific problem that would be primarily of interest to robotics-focused practitioners rather than the broader RL community.

    \end{enumerate}

    \item Answer to weakness: 
    
    \jypmodify{
    1. "Baselines."
    
    As detailed in related works (Section 2), there are several other ways to integrate time-reversal information.

    Some existing works exploit reversibility from goal states to enhance exploration of the agents, similar to what we would like to achieve through the time reversal guided reward shaping technique.
    Our method differs from them in that our proposed trajectory reversal augmentation technique leverages time reversal symmetry not only from goal states but globally for every transition in the trajectory, enabling a broader application of time symmetry across the entire state space.

    Other prior works are designed to avoid irreversible actions of the agent for safer exploration.
    One example is "learning a reset policy alongside the normal policy to prevent agents from entering non-reversible states, ensuring safety in exploration phase and achieving better training efficiency".
    Unlike their reset policy that sets the initial state as the ending state of the current policy and the goal state as the task's starting point, our method treats two reversible tasks independently, with initial and goal states defined separately for each task.
    Moreover, our method is orthogonal to theirs and can be integrated to enhance the training of their reset policy.}

    2. "Time reversal examples are a bit unclear." "You may be able to leverage ideas/definitions from [2] to motivate partial time reversibility."

    \jypmodify{
    % Thank you for highlighting the relevance of locally factored dynamics.
    We have updated our manuscript to recall state decomposition proposed by this work when we introduce the example of partial time reversal symmetry.
    The answer to your question in weakness\#2 is: Yes. 
    By our definition in Section 4.1, partial time reversal symmetry indicates that a subset of the whole state is reversible. 
    In the example of door opening/closing inward, it means that the door's trajectory can be reversed by some action.
    }

    \item Other comments:
    \begin{enumerate}
        \item The definition of partial time reversibility (line 149) reminds me of the definition of "locally factored dynamics" discussed in CoDA by Pitis et. al. [2]. Locally factored dynamics means that after taking an action, only a small number of components of the next state s' change. For instance, an object won't move unless the agent touches it, so if the agent and object are physically separated, the agent's dynamics are completely independent of the object's dynamics. This local structure allows Pitis et al. [2] to generate counterfactual transitions by swapping parts of next states across trajectories that share common context in the unaffected dimensions. You may be able to leverage ideas/definitions from [2] to motivate partial time reversibility. Followup works MoCoDA [3] and RoCoDA [4] may be of interest.
    \end{enumerate}

    \item Minor comments:
    \begin{enumerate}
        \item "existing work (see Related Work in Section 2) predominantly focuses on spatial symmetries, 28 such as translation, reflection, and rotation..." The authors might also mention augmentation methods that aim to improve robustness to noise (i.e. essentially all visual augmentation works, S4RL [5], and "sample enhancement" in [6])

        Answer: \jypmodify{
        Thank you for highlighting this important connection. 
        We have expanded the related work to explicitly include how data augmentation methods improve noise robustness and cited these two works as key examples.}

        \item Line 33: "speed of action execution" in this context, speed refers to the frequency at which actions are selected, right?

        Answer: \jypmodify{Yes, "the speed of action execution" is the frequency at which actions are selected. This is often controlled by a hyperparameter called "action repeat" in RL methods. A larger value of "action repeat" indicates a lower control frequency.}

        \item Figure 2: I should think of the reversal of this trajectories as reading the images in reverse from right to left, correct? Also, I suggest writing "Figure 2: Examples of reversible and irreversible trajectories" would help clarify what this figure is showing. (a) Reversible: ... (b) Irreversible ..." The juxtaposition of (a) and (b) made me think (b) was meant to represent the reversal of (a).

        Answer: \jypmodify{
        Thanks for this constructive suggestion. 
        We have updated our manuscript accordingly.}

        \item Line 105: the definitions of the dynamics function suggests stochastic dynamics, but does stochasticity interfere with reversibility?

        Answer: 
        \jypmodify{
        As defined in line 110, time reversal symmetry applies to probability distributions over transitions. 
        Consequently, stochastic dynamics does not interfere with reversibility, as it can remain statistically consistent under time reversal.}
        
        \item (not sure, notations) Line 111: The overhead arrow notation is not explicitly defined prior to using it.

        Answer: \jypmodify{To avoid confusion, we have explicitly added the following sentence at line 110 of our manuscript: $\cev{\cdot}$ denotes time reversal operation on $\mathcal{S}$ or $\mathcal{A}$.}

        \item Line 115: I think it's worth emphasizes somewhere that these sorts of symmetries frequently arise in the real world, so it's reasonable to assume these involutions exist.

        Answer: \jypmodify{
        Thank you for highlighting this important point. 
        As noted by Barkley et al. [2023] (cited at line 110), such time symmetries commonly emerge in physical systems. 
        We have now emphasized this point explicitly near line 115 in our manuscript.
        }

        \item (not sure, notations) When defining inverse dynamics models, it would help to unify notation a bit. For instance, $f_a$, $f_s$ could denote dynamics for inverse and forward dynamics models.
        
        Answer: 
        \jypmodify{
            Both $f_{\mathcal S}$ and $f_{\mathcal A}$ are used in Section 3 for involutions over states and actions.
            We choose to stick with the current notations for inverse and forward dynamics models ($h$ and $g$) to avoid misunderstanding.
        }
    
        \item Figures 5 and 6 would be much clearer if the results for each algorithm pair (TR vs. no TR)were plotted separately.
        
        Answer: \jypmodify{Due to page limit in the main text, we combine the results of all methods into a single plot. We will include separate plots for each algorithm pair (TR vs. no TR) in the appendix for better readability.}
    \end{enumerate}

    \item Questions:
    \begin{enumerate}
        \item "most reversed transitions are filtered out by the dynamics-consistent filter" Could you support this empirically? It'd be interesting to see how much is filtered out.

        Answer: \jypmodify{
            We empirically validate this point through quantitative analysis. 
            % First, in Figure 22 of our manuscript, trajectory reversal augmentation with filtering (blue curve) yields marginal gains (gap between the blue and black curves) for partially reversible tasks (e.g., door closing inward), under-performing compared to fully reversible tasks (e.g., door closing outward). 
            % This difference can support the hypothesis that most reversed transitions fail to pass filtering in partially reversible scenarios. 
            % Second, 
            We have tested our filtering method on the agent's saved replay buffer, which confirms that only 27.27$\%$ of transitions in door closing inward task pass filtering versus 63.13$\%$ for door closing outward task.}
            % Specifically in the scenario of door closing inward, passed reversed transitions mostly occur when the gripper is approaching and not touching the door. 
            % When the gripper is pushing the door to close it, most reversed transitions fail to pass filtering due to their violations of learned environment dynamics.}
            \hjsmodify{
            Specifically, when closing a door inward, transitions of the gripper approaching the door can be reverted, while the transitions of the gripper pushing the door fail to pass filtering due to their violations of learned environment dynamics.
            }

        \item "The training process alternates between two reversible tasks." Is this a critical part of the algorithm, or was this just chosen for convenience?
 
        Answer: \jypmodify{
            We would like to clarify that data collection (agent interacting with environments) in our method alternates between two tasks purely for implementation convenience.}
            % During agent update step, we sample transitions from replay buffers of both environments simultaneously, avoiding sequential single-task training.
            % This ensures joint optimization without introducing temporal bias toward either task.}
        \hjsmodify{It is expected to be more efficient to interact  with the two environments in parallel.
        During agent update step, we sample transitions from replay buffers of both environments simultaneously, and update all models with these transitions.
        }

        \item Do the authors have any sense of how the augmented data compares to additional policy-generated data? In particular, suppose we replaced the augmented data with additional data collected by the agent (and suppose we give the agent this data "for free" in that we don't count this data as additional timesteps).

        Answer: \jypmodify{
            Time reversal augmented data differs from policy generated data in quality and utility.
            One advantage of policy generated data is that it is 100$\%$ realistic and obeys environment dynamics, while time reversal augmented data, even after filtering, may not be fully dynamics-consistent.
            % Conversely, the advantage of time reversal augmented data lies in improving agent exploration, since these trajectories cover distinct regions of the state space, where policy generated data may rarely reach.
            % Take door opening and closing outward (Figure 9 and 10) as an example, closing the door from outward requires the agent to firstly reach the door at a distant position, then grasp the handle, and finally close the door.
            % In this case, time reversal augmented data from door opening outward task can provide crucial guidance, as trajectories of grasping the handle and opening the door outward can be reversed and thus reduce the agent's search space for door closing outward task.
            % This synergy is validated by the results shown in Figure 22 of our manuscript, where doubling the amount of policy generated data can not reach the performance of time reversal augmented data in this case.
        }
        \hjsmodify{Conversely, there are two advantages of time reversal augmented data.
        First, it could help improving agent exploration at the beginning of the training, since the trajectories from two tasks cover distinct regions of the state space.
        % Take door opening and closing outward (Figure 9 and 10) as an example, closing the door from outward requires the agent to firstly reach the door at a distant position, then grasp the handle, and finally close the door.
        % In this case, time reversal augmented data from door opening outward task can provide crucial guidance, as trajectories of grasping the handle and opening the door outward can be reversed and thus reduce the agent's search space for door closing outward task.
        This synergy is validated by the results shown in Figure 22 of our manuscript, where doubling the amount of policy generated data can not reach the performance of time reversal augmented data in this case.
        Second, the agent may converge at different speeds on the two tasks.
        A successful trajectory from one task can effectively guide the training for the other.}
    \end{enumerate}

    \item Limitations:
    \begin{enumerate}
        \item I think it's worth mentioning that this method assumes we know the task has time reversibility. I don't think this is a significant shortcoming though, since all data augmentation papers assume knowledge of some function that can transform observed data into additional training data (e.g. an augmentation function). This is just an inherent limitation of data augmentation methods. Corrado \& Hanna [1] and Pitis et al. [2] discuss this point.
    \end{enumerate}

    \item Answer to limitations:
    \jypmodify{
        % Thank you for highlighting this limitation. 
        We fully agree with this point and have explicitly included the following sentence in the limitations section of our manuscript. 
        "Like other data augmentation methods, our approach relies on prior knowledge of task structures—specifically, time reversal symmetry in our case."
    }
\end{itemize}

\subsection{Reviewer Pawe}
\jypmodify{Thank you for noting the quality and clarity of our work. 
We are happy that you recognize that the model design leading around our idea feels like the "shortest path". 
Below, we address each question thoroughly.}
\begin{itemize}
    \item Weakness: While the idea behind the work and the presented method are strong, the benchmarking and the results leave something to be desired. Particularly, evaluating on two somewhat simple simulated environments with some demonstration data already in the buffer makes the tasks accomplished incredibly simple. At the same time, from the plots, it seems that the performance improvements are not always clear – often there are significant overlaps in the error bars, and some more rigorous evaluations with more seeds, or more thorough investigation on a larger set of simulated and real environments, while not critical at this stage, will make this work significantly stronger.

    \item Questions:
    \begin{enumerate}
        \item (not sure) While the work only focuses on involutions created by forward and inverse dynamics models, could the authors think of some more interesting, maybe simpler involutions, which could take this beyond simple "negate the action sign" model? Perhaps even a learned action inverting model could give interesting results.

        Answer: 
        % \jypmodify{
        % % We appreciate the reviewer’s suggestion to explore alternative involutions beyond action negation. 

        % We would like to clarify that our method transcends this simplicity of "negate the action sign" model through two key innovations:

        % The first innovation is trajectory reversal augmentation with dynamics-aware filtering. 
        % By jointly training forward and inverse dynamics models, we can use the inverse dynamics model to generate actions for the reversed state pairs ($s_{t+1}, s_{t}$). 
        % Then these generated transitions are verified by the forward dynamics model so that dynamics-inconsistent ones are filtered out. 
        % We guess that "a learned action inverting model" proposed by the reviewer is what we call inverse dynamics model.
        
        % The second innovation is time reversal guided reward shaping.
        % This part can take advantage of partially reversible transitions.
        % As mentioned in our main text, we train a potential model using successful trajectories of task A and utilize this potential model to guide the agent training of task B.
        
        % In conclusion, both trajectory reversal augmentation with dynamics-aware filtering and time reversal guided reward shaping are not what purely "negating the action sign" can achieve.}

        \hjsmodify{
        We need to clarify that our method specifically learns an 'action inverting model' implemented via an inverse dynamics model.
        Unlike Barkley et al.'s approach of simply negating actions in reversed transitions—which is not always valid—our model derives reverted actions through a learned inverse dynamics.
        However, for transitions without full time reversal symmetry, the inverse dynamics model may still generate invalid actions.
        To address this, we introduce a forward dynamics model to filter out such invalid transitions.
        }

        \item (not sure, results) What would the results look like without the guiding demonstrations seeding the replay buffer? Would this method make a difference when exploring tabula rasa? If no, why not?

        Answer: 
        \jypmodify{
        In the sparse-reward setting, exploring tabula rasa is a very challenging task for the RL agent.
        Consequently, agent performance without demonstrations drops substantially, which is a key reason that we do not include these experiments in the manuscript.        
        On challenging tasks such as door opening/closing outward, nut assembly/disassembly, and block stacking/unstacking, the agents fail to make progress under sparse rewards alone. 
        However, on other tasks like door opening/closing inward and peg insertion/removal, the IQM of success rate (shown in the tables below) reveal that the performance gap between TR-DRL and baseline methods widens significantly without demonstrations, confirming that time reversal symmetry provides guidance and partially compensates for missing demonstration data.
        
        "Single-Task SAC": baseline; "+reversal aug": trajectory reversal augmentation with dynamics-aware filtering; "+reversal reward shaping": time reversal symmetry guided reward shaping.
        \begin{tabular}{c c c c c}
            \toprule
               \multirow{1}{*}{Task} & \multicolumn{4}{c}{Number of Environment Transitions} \\
              \multirow{1}{*}{Door opening inward}  & 50k & 100k & 150k & 200k\\
            \midrule
              Single-Task SAC & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} \\
            \midrule
              \makecell{+reversal aug} & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.18$\pm$0.36} \\
            \midrule
              \makecell{+reversal\\reward shaping} & \makecell{0.00$\pm$0.00} & \textbf{\makecell{0.13$\pm$0.26}} & \textbf{\makecell{0.31$\pm$0.41}} & \makecell{0.60$\pm$0.38} \\
            \midrule
              \makecell{Single-Task\\ TR-SAC \textbf{(Ours)}} & \makecell{0.00$\pm$0.00} & \makecell{0.11$\pm$0.22} & \makecell{0.26$\pm$0.37} & \textbf{\makecell{0.72$\pm$0.37}} \\
            \bottomrule
        \end{tabular}

        \begin{tabular}{c c c c c}
            \toprule
               \multirow{1}{*}{Task} & \multicolumn{4}{c}{Number of Environment Transitions} \\
              \multirow{1}{*}{Door closing inward}  & 50k & 100k & 150k & 200k\\
            \midrule
              Single-Task SAC & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.05$\pm$0.09} & \makecell{0.19$\pm$0.36} \\
            \midrule
              \makecell{+reversal aug} & \makecell{0.00$\pm$0.00} & \makecell{0.20$\pm$0.40} & \makecell{0.20$\pm$0.40} & \makecell{0.37$\pm$0.45} \\
            \midrule
              \makecell{+reversal\\reward shaping} & \makecell{0.03$\pm$0.06} & \textbf{\makecell{0.29$\pm$0.28}} & \makecell{0.46$\pm$0.38} & \makecell{0.69$\pm$0.35} \\
            \midrule
              \makecell{Single-Task\\ TR-SAC \textbf{(Ours)}} & \makecell{0.02$\pm$0.03} & \makecell{0.29$\pm$0.35} & \textbf{\makecell{0.55$\pm$0.41}} & \textbf{\makecell{0.77$\pm$0.30}} \\
            \bottomrule
        \end{tabular}

        \begin{tabular}{c c c c c}
            \toprule
               \multirow{1}{*}{Task} & \multicolumn{4}{c}{Number of Environment Transitions} \\
              \multirow{1}{*}{Peg Insertion}  & 50k & 100k & 150k & 200k\\
            \midrule
              Single-Task SAC & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.00$\pm$0.00} & \makecell{0.23$\pm$0.24} \\
            \midrule
              \makecell{+reversal aug} & \makecell{0.05$\pm$0.09} & \makecell{0.37$\pm$0.33} & \makecell{0.58$\pm$0.37} & \makecell{0.95$\pm$0.07} \\
            \midrule
              \makecell{+reversal\\reward shaping} & \makecell{0.07$\pm$0.09} & \makecell{0.37$\pm$0.44} & \makecell{0.55$\pm$0.45} & \makecell{0.75$\pm$0.38} \\
            \midrule
              \makecell{Single-Task\\ TR-SAC \textbf{(Ours)}} & \textbf{\makecell{0.16$\pm$0.16}} & \textbf{\makecell{0.50$\pm$0.39}} & \textbf{\makecell{0.91$\pm$0.07}} & \textbf{\makecell{1.00$\pm$0.00}} \\
            \bottomrule
        \end{tabular}

        \begin{tabular}{c c c c c}
            \toprule
               \multirow{1}{*}{Task} & \multicolumn{4}{c}{Number of Environment Transitions} \\
              \multirow{1}{*}{Peg Removal}  & 50k & 100k & 150k & 200k\\
            \midrule
              Single-Task SAC & \makecell{0.00$\pm$0.00} & \makecell{0.09$\pm$0.17} & \makecell{0.27$\pm$0.39} & \makecell{0.64$\pm$0.37} \\
            \midrule
              \makecell{+reversal aug} & \textbf{\makecell{0.25$\pm$0.26}} & \makecell{0.81$\pm$0.31} & \textbf{\makecell{1.00$\pm$0.00}} & \textbf{\makecell{1.00$\pm$0.00}} \\
            \midrule
              \makecell{+reversal\\reward shaping} & \makecell{0.00$\pm$0.00} & \makecell{0.23$\pm$0.39} & \makecell{0.52$\pm$0.44} & \makecell{0.63$\pm$0.45} \\
            \midrule
              \makecell{Single-Task\\ TR-SAC \textbf{(Ours)}} & \makecell{0.08$\pm$0.10} & \textbf{\makecell{0.86$\pm$0.15}} & \textbf{\makecell{1.00$\pm$0.00}} & \textbf{\makecell{1.00$\pm$0.00}} \\
            \bottomrule
        \end{tabular}
        }

        % |Task|Number of Transitions |50k|100k|150k|200k|
        % |:----------------- | :-------------------------------- | :------ | :------ | :------ | :------ |
        % |**Door opening inward**||||||
        % |Single-Task SAC|  | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  |
        % |+ reversal aug| | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  | `0.18±0.36`  |
        % |+ reversal reward shaping || `0.00±0.00`  | **`0.13±0.26`** | **`0.31±0.41`** | `0.60±0.38`  |
        % |Single-Task TR-SAC **(Ours)**|| `0.00±0.00`  | `0.11±0.22`  | `0.26±0.37`  | **`0.72±0.37`** |
        % |**Door closing inward**||||||
        % |Single-Task SAC|  | `0.00±0.00`  | `0.00±0.00`  | `0.05±0.09`  | `0.19±0.36`  |
        % |+ reversal aug| | `0.00±0.00`  | `0.20±0.40`  | `0.20±0.40`  | `0.37±0.45`  |
        % |+ reversal reward shaping || `0.03±0.06`  | **`0.29±0.28`** | `0.46±0.38` | `0.69±0.35`  |
        % |Single-Task TR-SAC **(Ours)**|| `0.02±0.03`  | `0.29±0.35`  | **`0.55±0.41`**  | **`0.77±0.30`** |
        % |**Peg Insertion**||||||
        % |Single-Task SAC|  | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  | `0.23±0.24`  |
        % |+ reversal aug| | `0.05±0.09`  | `0.37±0.33`  | `0.58±0.37`  | `0.95±0.07`  |
        % |+ reversal reward shaping || `0.07±0.09`  | `0.37±0.44` | `0.55±0.45` | `0.75±0.38`  |
        % |Single-Task TR-SAC **(Ours)**|| **`0.16±0.16`**  | **`0.50±0.39`**  | **`0.91±0.07`**  | **`1.00±0.00`** |
        % |**Peg Removal**||||||
        % |Single-Task SAC|  | `0.00±0.00`  | `0.09±0.17`  | `0.27±0.39`  | `0.64±0.37`  |
        % |+ reversal aug| | **`0.25±0.26`**  | `0.81±0.31`  | **`1.00±0.00`**  | **`1.00±0.00`**  |
        % |+ reversal reward shaping || `0.00±0.00`  | `0.23±0.39` | `0.52±0.44` | `0.63±0.45`  |
        % |Single-Task TR-SAC **(Ours)**|| `0.08±0.10`  | **`0.86±0.15`**  | **`1.00±0.00`**  | **`1.00±0.00`** |
        
        
        % \jypmodify{
        % To further validate the effectiveness of our proposed techniques, we have also conducted additional experiments on MT50 with random goals, dense rewards, and no demonstrations. 
        % Building upon MOORE [1], a state-of-the-art multi-task reinforcement learning method, we integrated our proposed techniques, which is orthogonal to their network architecture innovation. 
        % This seamless integration enables direct comparisons against vanilla MOORE. 
        % Results demonstrate consistent performance gains, confirming that our approach maintains effectiveness even in the absence of demonstrations.

        % Comparison of MOORE and TR-MOORE on Meta-World-V2 MT50 with random goals (MT50-rand).
        % \begin{tabular}{c|c c c c c c c}
        %    Total Env Steps & 5M & 10M & 15M & 20M & 30M & 40M & 50M \\
        % \hline
        %    \makecell{MOORE\\(reproduced\\5 seeds)} & \makecell{28.2\\$\pm$1.8} & \makecell{38.2\\$\pm$1.9} & \makecell{44.3\\$\pm$2.3} & \makecell{47.9\\$\pm$3.5} & \makecell{50.4\\$\pm$2.3} & \makecell{51.6\\$\pm$3.3} & \makecell{52.9\\$\pm$3.9} \\
        % \hline
        %    \makecell{TR-MOORE\\(5 seeds)} & \textbf{\makecell{41.1\\$\pm$1.0}} & \textbf{\makecell{50.9\\$\pm$1.8}} & \textbf{\makecell{52.6\\$\pm$1.4}} & \textbf{\makecell{54.2\\$\pm$2.2}} & \textbf{\makecell{55.5\\$\pm$2.9}} & \textbf{\makecell{57.1\\$\pm$2.4}} & \textbf{\makecell{58.7\\$\pm$2.5}} \\
        % \end{tabular}
        
        % [1] Hendawy, et al. "Multi-Task Reinforcement Learning with Mixture of Orthogonal Experts." https://arxiv.org/abs/2311.11385}

    \end{enumerate}

    \item Limitations: While the authors mention the lack of real world experiments, there are further limitations beyond that. Particularly, the method currently is limited to quasi-static environments, and would be hard to extend to domains such as video games or self-driving because the environments are generally dynamic and there is a definite "forward arrow of time" in such settings.

    Answer: \jypmodify{
        We fully agree with your observation regarding our method’s current limitations.
        % in dynamic environments like video games or self-driving scenarios. 
        We will update this limitation in the revised manuscript.
        % We will clearly articulate this limitation in the revised manuscript, discussing how the strict "forward arrow of time" in such settings conflicts with our core assumption of time reversibility. 
        % Thank you for raising this critical point.
    }

    \item Paper formatting concerns: Fonts on images can be small and hard to read on print. Please try to ensure the image fonts at least match the paper font size.

    Answer: \jypmodify{
        We appreciate your feedback.
        % regarding legibility of text in figures. 
        % In response, 
        We will increase image font sizes to improve readability in the final version.
        % Thank you for this important suggestion.
    }
\end{itemize}

\subsection{Reviewer dzfv}
\jypmodify{We sincerely appreciate your positive evaluation, especially noting the intuitiveness of our approach. 
In response to your observations about weaknesses, below we provide answers in detail.}

\begin{itemize}
    \item Weakness:
    \begin{enumerate}
        \item A key question here is whether this method passes the bang-for-buck threshold. In order to use this method, you need to learn forward and inverse dynamics models, significantly adding to the compute complexity of the alg. There is a benefit to doing so, but it may not be enough on its own to warrant learning those extra models. On the other hand, there are probably plenty of situations where folks are already learning those dynamics models and the method would definitely make sense there.

        Answer: 
        \jypmodify{We agree that learning forward and inverse dynamics models has additional computational cost but emphasize that superior sample efficiency is a critical goal in deep RL. 
        Like common techniques such as data augmentation or auxiliary losses, this added computation directly enables efficient learning with fewer samples and better final performance. 
        Furthermore, our method seamlessly integrates with existing approaches that have already trained dynamics models, offering enhanced performance without incremental computational cost in such cases.}
        
        \item (not sure about the example) I can't help but wonder if there might be more effective and sophisticated ways of leveraging the time reversal symmetry. There should be some systems for which time reversal should yield a 2x speedup. Are there ways to maybe incorporate time reversal directly into the neural model? Not clear, but interesting.

        Answer:
        \jypmodify{We appreciate your insightful suggestion about sophisticated ways of leveraging time reversal symmetry and we agree that it is an interesting topic.}
        % Specifically, as proposed by the reviewer, incorporating time reversal directly into the neural model is a promising future direction in this research area, similar to steerable CNN handling spatial symmetry like rotation equivariance.
        % For example, imagine a model trained on data from door opening task. 
        % During inference, presenting it with an initial state of an open door and the instruction of "closing the door" would automatically generate actions to close it.
        \hjsmodify{One possible approach is to incorporate the temporal symmetry into the neural network architecture design, similar to steerable CNN handling spatial symmetry like rotation equivariance.}
        \jypmodify{
        % Such model that has inherent time reversal symmetry could significantly enhance sample efficiency.
        Moreover, we suspect that the 2x speedup may be too optimistic.
        This would require idealized conditions rarely met in practice, including perfectly reversible dynamics and accurate backward policy execution.
        }
    \end{enumerate}

    \item Limitation: I think complexity is a limitation. I also think that there there might be more effective ways to do this beyond data augmentation and dense rewardifying.
\end{itemize}


\section{Markdown}
\subsection{Reviewer fKuw}
Thank you for indicating our contributions and providing thoughtful feedback on our work. 
In this work, we focus on robotics tasks with time reversal symmetry, and evaluate our proposed method in simulation. 
We definitely agree that applying our approach in a real-world setting is an important step to prove the effectiveness of our method for solving those time-symmetric robotics tasks.
And it is an interesting direction to learn the temporal symmetry if it does not obviously exist in tasks.
We leave the real-world experiments and learning temporal symmetry as future work.
Below, we answer each question in detail.

**Q1**. "Can the time reversal..."

We would like to clarify that our method exploits two types of symmetry: full time reversal symmetry (FTR) and partial time reversal symmetry (PTR). 
Peg insertion/removal and door opening/closing inward are examples of FTR and PTR task pairs respectively.
In door opening/closing inward, most reversed transitions are filtered out by the dynamics-consistent filter, since the agent cannot reverse the action (i.e., from "push the door" to "grasp the handle and pull the door") without first grasping the handle.
The detailed examples of partial reversibility can be found in Example 2 of Section 4.1.
We design a time reversal reward shaping mechanism to handle these partially reversible transitions.
A potential model is trained with successful trajectories of task A and used to guide the agent training of task B through potential-based reward shaping, as detailed in Section 4.3.

**Q2**. "Given that the paper..."

As stated at the beginning of the response, we admit the significance of real-world experiments and leave it as future work.
Considering the difficulties of conducting RL directly under real-world setting, a common practice is to train the policy with RL in simulation and deploy the policy in real-world by solving the sim-to-real gap.
Our approach can effectively facilitate the learning process during the simulation phase.

**Q3**. "In partially reversible tasks..."

For tasks where only subsets of states exhibit time reversal symmetry, reversed trajectories obtained from trajectory reversal augmentation often violate true environment dynamics, leading to low quality data that may even hurt agent training.
Instead, our method leverages time reversal guided reward shaping to exploit the partial reversibility.
Intuitively, for a high-reward trajectory from one task (door from open to closed), if a trajectory from another task can achieve the reversed object states (door from closed to open), it should likewise receive a high reward.
This motivates us to employ reward shaping to guide the RL agent with these partially reversible transitions, as detailed in Section 4.3.
Furthermore, we choose to use potential-based reward shaping as it preserves policy optimality and train a potential model so that we can fully utilize all successful trajectories.

\subsection{Reviewer TdWt}
Thank you for summarizing our work and providing thoughtful feedback that helps us strengthen both the presentation and technical depth of our paper.
Below we answer your questions in detail.

**Weakness1**. "Baselines..."

As detailed in related works (Section 2), there are several other ways to integrate time-reversal information.

Some existing works exploit reversibility from goal states to enhance exploration of the agents, similar to what we would like to achieve through the time reversal guided reward shaping technique.
Our method differs from them in that our proposed trajectory reversal augmentation technique leverages time reversal symmetry not only from goal states but globally for every transition in the trajectory, enabling a broader application of time symmetry across the entire state space.

Other prior works are designed to avoid irreversible actions of the agent for safer exploration.
One example is "learning a reset policy alongside the normal policy to prevent agents from entering non-reversible states, ensuring safety in exploration phase and achieving better training efficiency".
Unlike their reset policy that sets the initial state as the ending state of the current policy and the goal state as the task's starting point, our method treats two reversible tasks independently, with initial and goal states defined separately for each task.
Moreover, our method is orthogonal to theirs and can be integrated to enhance the training of their reset policy.

**Weakness2**. "Time reversal examples..."

We have updated our manuscript to recall state decomposition proposed by this work when we introduce the example of partial time reversal symmetry.
The answer to your question in **Weakness2** is: Yes. 
By our definition in Section 4.1, partial time reversal symmetry indicates that a subset of the whole state is reversible. 
In the example of door opening/closing inward, it means that the door's trajectory can be reversed by some action.

**Minor1**. "existing work..."

Thank you for highlighting this important connection. 
We have expanded the related work to explicitly include how data augmentation methods improve noise robustness and cited these two works as key examples.

**Minor2**. "Line 33:..."

Yes, "the speed of action execution" is the frequency at which actions are selected. 
This is often controlled by a hyperparameter called "action repeat" in RL methods. 
A larger value of "action repeat" indicates a lower control frequency.

**Minor3**. "Figure 2:..."

Thanks for this constructive suggestion. 
We have updated our manuscript accordingly.

**Minor4**. "Line 105:..."

As defined in line 110, time reversal symmetry applies to probability distributions over transitions. 
Consequently, stochastic dynamics does not interfere with reversibility, as it can remain statistically consistent under time reversal.

**Minor5**. "Line 111:..."

To avoid confusion, we have explicitly defined the overhead arrow notation as time reversal operation on $\mathcal{S}$ or $\mathcal{A}$ at line 110 of our manuscript.

**Minor6**. "Line 115:..."

Thank you for highlighting this important point. 
As noted by Barkley et al. (cited at line 110), such time symmetries commonly emerge in physical systems. 
We have now emphasized this point explicitly near line 115 in our manuscript.

**Minor7**. "When defining..."

Both $f_{\mathcal S}$ and $f_{\mathcal A}$ are used in Section 3 for involutions over states and actions.
We choose to stick with the current notations for inverse and forward dynamics models ($h$ and $g$) to avoid misunderstanding.

**Minor8**. "Figures 5 and 6..."

Due to page limit in the main text, we combine the results of all methods into a single plot. 
We will include separate plots for each algorithm pair (TR vs. no TR) in the appendix for better readability.

**Question1**. "most reversed transitions..."

We empirically validate this point through quantitative analysis. 
We have tested our filtering method on the agent's saved replay buffer, which confirms that only 27.27\% of transitions in door closing inward task pass filtering versus 63.13\% for door closing outward task.
Specifically, when closing a door inward, transitions of the gripper approaching the door can be reverted, while the transitions of the gripper pushing the door fail to pass filtering due to their violations of learned environment dynamics.

**Question2**. "The training process alternates..."

We would like to clarify that data collection (agent interacting with environments) in our method alternates between two tasks purely for implementation convenience.
It is expected to be more efficient to interact with the two environments in parallel.
During agent update step, we sample transitions from replay buffers of both environments simultaneously, and update all models with these transitions.

**Question3**. "Do the authors..."

Time reversal augmented data differs from policy generated data in quality and utility.
One advantage of policy generated data is that it is 100\% realistic and obeys environment dynamics, while time reversal augmented data, even after filtering, may not be fully dynamics-consistent.
Conversely, there are two advantages of time reversal augmented data.
First, it could help improving agent exploration at the beginning of the training, since the trajectories from two tasks cover distinct regions of the state space.
This synergy is validated by the results shown in Figure 22 of our manuscript, where doubling the amount of policy generated data can not reach the performance of time reversal augmented data in this case.
Second, the agent may converge at different speeds on the two tasks.
A successful trajectory from one task can effectively guide the training for the other.

**Limitations**. "Yes, but I think it's worth mentioning..."

We fully agree with this point and have explicitly included the following sentence in the limitations section of our manuscript. 
"Like other data augmentation methods, our approach relies on prior knowledge of task structures—specifically, time reversal symmetry in our case."

\subsection{Reviewer Pawe}
Thank you for noting the quality and clarity of our work. 
We are happy that you recognize that the model design leading around our idea feels like the "shortest path". 
Below, we address each question thoroughly.

**Q1**. "While the work..."

We need to clarify that our method specifically learns an 'action inverting model' implemented via an inverse dynamics model.
Unlike Barkley et al.'s approach [1] of simply negating actions in reversed transitions—which is not always valid—our model derives reverted actions through a learned inverse dynamics.
However, for transitions without full time reversal symmetry, the inverse dynamics model may still generate invalid actions.
To address this, we introduce a forward dynamics model to filter out such invalid transitions.        

**Q2**. "What would the results..."

In the sparse-reward setting, exploring tabula rasa is a very challenging task for the RL agent.
Consequently, agent performance without demonstrations drops substantially, which is a key reason that we do not include these experiments in the manuscript.
On challenging tasks such as door opening/closing outward, nut assembly/disassembly, and block stacking/unstacking, the agents fail to make progress under sparse rewards alone. 
However, on other tasks like door opening/closing inward and peg insertion/removal, , the IQM of success rate (shown in the tables below) reveal that the performance gap between TR-DRL and baseline methods widens significantly without demonstrations, confirming that time reversal symmetry provides guidance and partially compensates for missing demonstration data.
        
 "Single-Task SAC": baseline; "+reversal aug": trajectory reversal augmentation with dynamics-aware filtering; "+reversal reward shaping": time reversal symmetry guided reward shaping.
|Task|Number of Transitions |50k|100k|150k|200k|
|:----------------- | :-------------------------------- | :------ | :------ | :------ | :------ |
|**Door opening inward**||||||
|Single-Task SAC|  | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  |
|+ reversal aug| | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  | `0.18±0.36`  |
|+ reversal reward shaping || `0.00±0.00`  | **`0.13±0.26`** | **`0.31±0.41`** | `0.60±0.38`  |
|Single-Task TR-SAC **(Ours)**|| `0.00±0.00`  | `0.11±0.22`  | `0.26±0.37`  | **`0.72±0.37`** |
|**Door closing inward**||||||
|Single-Task SAC|  | `0.00±0.00`  | `0.00±0.00`  | `0.05±0.09`  | `0.19±0.36`  |
|+ reversal aug| | `0.00±0.00`  | `0.20±0.40`  | `0.20±0.40`  | `0.37±0.45`  |
|+ reversal reward shaping || `0.03±0.06`  | **`0.29±0.28`** | `0.46±0.38` | `0.69±0.35`  |
|Single-Task TR-SAC **(Ours)**|| `0.02±0.03`  | `0.29±0.35`  | **`0.55±0.41`**  | **`0.77±0.30`** |
|**Peg Insertion**||||||
|Single-Task SAC|  | `0.00±0.00`  | `0.00±0.00`  | `0.00±0.00`  | `0.23±0.24`  |
|+ reversal aug| | `0.05±0.09`  | `0.37±0.33`  | `0.58±0.37`  | `0.95±0.07`  |
|+ reversal reward shaping || `0.07±0.09`  | `0.37±0.44` | `0.55±0.45` | `0.75±0.38`  |
|Single-Task TR-SAC **(Ours)**|| **`0.16±0.16`**  | **`0.50±0.39`**  | **`0.91±0.07`**  | **`1.00±0.00`** |
|**Peg Removal**||||||
|Single-Task SAC|  | `0.00±0.00`  | `0.09±0.17`  | `0.27±0.39`  | `0.64±0.37`  |
|+ reversal aug| | **`0.25±0.26`**  | `0.81±0.31`  | **`1.00±0.00`**  | **`1.00±0.00`**  |
|+ reversal reward shaping || `0.00±0.00`  | `0.23±0.39` | `0.52±0.44` | `0.63±0.45`  |
|Single-Task TR-SAC **(Ours)**|| `0.08±0.10`  | **`0.86±0.15`**  | **`1.00±0.00`**  | **`1.00±0.00`** |

[1]. Barkley et al. "An Investigation of Time Reversal Symmetry in Reinforcement Learning." https://arxiv.org/abs/2311.17008

\subsection{Reviewer dzfv}
We sincerely appreciate your positive evaluation, especially noting the intuitiveness of our approach.
In response to your observations about weaknesses, below we provide answers in detail.

**Weakness1**. "A key question here..."

We agree that learning forward and inverse dynamics models has additional computational cost but emphasize that superior sample efficiency is a critical goal in deep RL. 
Like common techniques such as data augmentation or auxiliary losses, this added computation directly enables efficient learning with fewer samples and better final performance. 
Furthermore, our method seamlessly integrates with existing approaches that have already trained dynamics models, offering enhanced performance without incremental computational cost in such cases.

**Weakness2**. "I can't help but wonder..."

We appreciate your insightful suggestion about sophisticated ways of leveraging time reversal symmetry and we agree that it is an interesting topic.
One possible approach is to incorporate the temporal symmetry into the neural network architecture design, similar to steerable CNNs handling spatial symmetry like rotation equivariance.
Moreover, we suspect that the 2x speedup may be too optimistic.
This would require idealized conditions rarely met in practice, including perfectly reversible dynamics and accurate backward policy execution.
        
